Structure Invariant Transformation for better Adversarial Transferability

Given the severe vulnerability of Deep Neural Networks (DNNs) against adversarial examples, there is an urgent need for an effective adversarial attack to identify the deficiencies of DNNs in security-sensitive applications. As one of the prevalent black-box adversarial attacks, the existing transfer-based attacks still cannot achieve comparable performance with the white-box attacks. Among these, input transformation based attacks have shown remarkable effectiveness in boosting transferability. In this work, we find that the existing input transformation based attacks transform the input image globally, resulting in limited diversity of the transformed images. We postulate that the more diverse transformed images result in better transferability. Thus, we investigate how to locally apply various transformations onto the input image to improve such diversity while preserving the structure of image. To this end, we propose a novel input transformation based attack, called Structure Invariant Attack (SIA), which applies a random image transformation onto each image block to craft a set of diverse images for gradient calculation. Extensive experiments on the standard ImageNet dataset demonstrate that SIA exhibits much better transferability than the existing SOTA input transformation based attacks on CNN-based and transformer-based models, showing its generality and superiority in boosting transferability. Code is available at https://github.com/xiaosen-wang/SIT.

==> figs/ablation_combination.tex <==
\begin{figure}
    \centering
    \includegraphics[scale=0.4]{figs/pdf/pos_ablation_combination.pdf}
    \caption{The classification accuracy (\%) of various deep models on the adversarial examples generated by \name using one or two transformations. The adversarial examples are generated on Resnet18 and tested on the other seven models.}
    \label{fig:single_model_attack}
\end{figure}

==> figs/ablation_remove.tex <==
\begin{figure}
    \centering
    \includegraphics[scale=0.5]{figs/pdf/neg_ablation_combination.pdf}
    \caption{The classification accuracy (\%) of various deep models on the adversarial examples generated by \name after removing one or two transformations. The adversarial examples are generated on Resnet18 and tested on the other seven models.}
    \label{fig:single_model_attack}
\end{figure}
